Family of Controllers for Attitude Synchronization on the Sphere

In this paper we study a family of controllers that guarantees attitude synchronization for a network of elements in the unit sphere domain, i.e. $\mathcal{S}^2$. We propose distributed continuous controllers for elements whose dynamics are controllable (i.e. control with torque as command), and which can be implemented by each individual agent without the need of a common global orientation frame among the network, i.e. it requires only local information that can be measured by each individual agent from its own orientation frame. The controllers are specified according to arbitrary distance functions in $\mathcal{S}^2$, and we provide conditions on those distance functions that guarantee that i) a synchronized network of agents is locally asymptotically stable for an arbitrary network graph; ii) a synchronized network can be achieved for almost all initial conditions in a tree graph network. We also study the equilibria configurations that come with specific types of network graphs. The proposed strategies can be used in attitude synchronization of swarms of fully actuated rigid bodies, such as satellites.

==> Contents/FrontMatter.tex <==
%\runtitle{Insert a suggested running title}  % Running title for regular 
                                              % papers but only if the title  
                                              % is over 5 words. Running title 
                                              % is not shown in output.


%%Title, preferably not more than 10 words
\title{Family of Controllers for Attitude Synchronization \\ on the Sphere\thanksref{footnoteinfo}} % .

\thanks[footnoteinfo]{ %
This project has received funding from the European Union's Horizon 2020 Research and Innovation Programme under the Grant Agreement No.~644128 (AEROWORKS). This work was also supported by the Swedish Research Council (VR).
}

% \thanks[footnoteinfo]{This paper was not presented at any IFAC  meeting.}

% Add the e-mail address (ead) as shown
\author[1]{Pedro~O.~Pereira}\ead{ppereira@kth.se} \, and 
\author[1]{Dimos~V.~Dimarogonas}\ead{dimos@kth.se}

% Please full addresses here
\address[1]{ACCESS Linnaeus Center and KTH Centre for Automomous Systems, School of Electrical Engineering, KTH Royal Institute of Technology, Stockholm, Sweden.}
%\address[2]{KTH Centre for Automomous Systems, School of Electrical Engineering, KTH Royal Institute of Technology, Stockholm, Sweden.}


% Five to ten keywords, chosen from the IFAC keyword list or with the help of the Automatica keyword wizard
%\begin{keyword}
%
%\end{keyword}




==> Contents/Solution.tex <==
Consider an arbitrary metric between unit vectors $d(\nmbi{1},\nmbi{2}): \mathcal{S}^{3} \times \mathcal{S}^{3} \rightarrow \mathbb{R}_{0}^{+}$, satisfying
%
\begin{enumerate}
	\item $d(\nmbi{1},\nmbi{2}) \ge 0$,
	\item $d(\nmbi{1},\nmbi{2}) = 0 \Leftrightarrow \nmbi{1} = \nmbi{2}$,
	\item $d(\nmbi{1},\nmbi{2}) = d(\nmbi{2},\nmbi{1})$.
	% \item $0 < d(\nmbi{1},\nmbi{2})  < d^{\sss{\max}}$, for all $\nmbi{1} \ne \pm \nmbi{2}$
\end{enumerate}
%
%The triangular inequality $d(\nmbi{1},\nmb_{\sss{3}}) \le d(\nmbi{1},\nmbi{2}) + d(\nmbi{2},\nmb_{\sss{3}})$ does not need to be satisfied. 
%
In addition, we may require the distance between unit vectors to be maximum when those unit vectors are diametrically opposed
%
\begin{enumerate}
	\setcounter{enumi}{3}
	\item $d(\nmbi{1},-\nmbi{1}) = \underset{\vmb_1,\vmb_2 \in \Omega}{\max} \, d(\vmb_1,\vmb_2)  \triangleq d^{\sss{\max}}$ for all $\nmbi{1}$.
\end{enumerate}

We want to exploit the result in Proposition~\cite{prop:Bdefinitepositive}, which is why we impose the following \emph{natural} condition,
%
\begin{align}
	\sk{\nmb_1}
	\frac{\partial d(\nmbi{1},\nmbi{2})}{\partial \nmbi{1}} 
	= 
	-
	\sk{\nmb_2}
	\frac{\partial d(\nmbi{1},\nmbi{2})}{\partial \nmbi{2}},
	\label{eq:MetricProperty}
\end{align}
%
where $\frac{\partial d(\nmbi{1},\nmbi{2})}{\partial \nmbi{1}}$ is the gradient of the metric w.r.t. the first argument.
%

By invoking uniqueness of solutions to the PDE~\eqref{eq:MetricProperty} and by verifying that $d(\nmb_1\tp\nmb_2)$ satisfies~\eqref{eq:MetricProperty}, one can conclude $d(\nmb_1\tp \nmb_2)$ is the only type of metric that satisfies~\eqref{eq:MetricProperty}.

As such, we restrict ourselves to metrics of the type
%
\begin{align}
	d(\nmb_1,\nmb_2) = d(\nmb_1\tp\nmb_2),
\end{align}
%
which are invariant to rotation of their arguments, i.e. $d(\Rmat \nmb_1, \Rmat\nmb_2) = d(\nmb_1\tp\xmb_2)$, and this property will guarantee that the proposed controllers can be implemented without the need of a common inertial attitude frame.

A simple metric is $d_{\theta}(\nmbi{1},\nmbi{2}) : \mathcal{S}^{3} \times \mathcal{S}^{3} \rightarrow [0,\pi]$
%
\begin{align}
	d_{\theta}(\nmbi{1},\nmbi{2}) = \arccos(\nmbi{1}\tp\nmbi{2})
\end{align}
%
whose gradient is given by
%
\begin{align}
	\frac{\partial d(\nmbi{1},\nmbi{2})} {\partial \nmbi{1}} 
	= 
	- \frac{1}{\sqrt{1 - (\nmbi{1}\tp\nmbi{2})^2}} \nmbi{2}
	= 
	- \frac{1}{\norm{\sk{\nmbi{1}}\nmbi{2}}} \nmbi{2}.
	\label{eq:BasicMetricGradient}
\end{align}
%

We will focus attention on an arbitrary metrics $d(\nmbi{1},\nmbi{2})$ that can be obtained from  $d_{\theta}(\nmbi{1},\nmbi{2})$ by means of an increasing function $f(s):\mathbb{R}_{0}^{+} \rightarrow \mathbb{R}_{0}^{+}$, i.e.
%
\begin{align}
	d(\nmbi{1},\nmbi{2}) = f(d_{\theta}(\nmbi{1},\nmbi{2})).
\end{align}
%
which means the gradient of an arbitrary metric can be obtained from~\eqref{eq:BasicMetricGradient} as
%
\begin{align}
	\frac{\partial d(\nmbi{1},\nmbi{2})}{\partial \nmbi{1}} 
	= 
	f'(d_{\theta}(\nmbi{1},\nmbi{2})) 
	\frac{\partial d_{\theta}(\nmbi{1},\nmbi{2})}{\partial \nmbi{1}}
	= 
	- \frac{f'(d_{\theta}(\nmbi{1},\nmbi{2})) }{\norm{\sk{\nmbi{1}}\nmbi{2}}} \nmbi{2}.
	\label{eq:ArbitraryMetricGradient}
\end{align}

Nonetheless, requiring $f$ to be increasing can be lifted under certain conditions.

We then proposed the following distributed control law,
%
\begin{align}
	\Omi{V_i} 
	& =
	- \sum_{j \in \mathcal{N}_{\sss{V_i}}} 
	\sk{\nmbi{V_i}} \frac{\partial d_{ij}(\nmbi{V_i},\nmbi{V_j})}{\partial \nmbi{V_i}}	
	\\
	& =
	\sum_{j \in \mathcal{N}_{\sss{V_i}}} 
	f_{ij}'(d_{\theta}(\nmbi{V_i},\nmbi{V_j}))
	\frac{ \sk{\nmbi{V_i}}\nmbi{V_j} }{\norm{\sk{\nmbi{V_i}}\nmbi{V_j}}},
	\label{eq:DistributedControlLaw}
\end{align}
%
where the used metric can be different for each agent and for each edge. 

\begin{thm}
	\label{thm:HalfSphereDomainExtended}
	Consider a directed connected graph for a group of unit vectors with kinematics~\eqref{eq:UnitVectorKinematics}. Assume the control law is given by~\eqref{eq:DistributedControlLaw} with a metric that satisfies
	%
	\begin{align}
			\frac{f_{ij}'(d_{\theta}(\nmbi{1},\nmbi{2})) }{\norm{\sk{\nmbi{1}}\nmbi{2}}} \ge k > 0 \quad \forall \nmbi{1}\tp\nmbi{2} \ge 0 ,
			\label{eq:LimitCondition2}
	\end{align}
	%
	for all $ i \in \{1,\cdots,N\}$ and all $\forall j \in \{1,\cdots,M\}$. If
	\begin{align}
		\underset{i,j}{\min}( \nmbi{E_i}\tp(0)\nmbi{E_j}(0)) > 0,
	\end{align}
	%
	then all unit vectors asymptotically converge to each other.
\end{thm}

\begin{proof}
	Consider the following the set
	%
	\begin{align}
		C 
		& =
		\left\{
			(i,j) \in V \times V: 
			\frac{\nmb_i\tp\nmb_j}{\nmb_k \tp \nmb_l } \le 1
			\quad 
			\forall (k,l) \in V \times V
		\right\}.
		\label{eq:CSetDef2}
	\end{align}
	%	
	which contains all the pairs of agents that minimize their unit vector inner product (we work under the assumption that $\nmb_i\tp \nmb_j >0$ for $(i,j) \in V \times V$). Notice that $C\backslash \{V\times V\}  = \emptyset$ if and only if all unit vectors are the same. 
	This set can contain multiple pairs and we construct a smaller set, namely 
	%
	\begin{align}
		\bar{C}
		=
		C \backslash
		\left\{
			(i,j) \in C : 
			\nmb_i\tp \nmb_k = 1 \forall k \in \mathcal{N}_i
			\wedge
			\nmb_j\tp \nmb_l = 1 \forall l \in \mathcal{N}_j
		\right\}
	\end{align}
	%
	which contains all elements of $C$, i.e. $\bar{C} \subset C$, except the pairs $(i,j)$ whose neighbors of agent~$i$ are all aligned with $i$ and  whose neighbors of agent~$j$ are all aligned with $j$ (for these pairs, $\bm{\omega}_i$ and $\bm{\omega}_j$ will be $\zvec$ at the time instant where all neighbors of agent~$i$/$j$ are aligned with agent~$i$/$j$). Notice that both $C$ and $\bar{C}$ can change with time and that $\bar{C}$ is always non-empty as long as the graph is connected and $C\backslash \{V\times V\}  \ne \emptyset$, i.e if not all agents are aligned.
	
	Given these sets, consider a pair $(i,j)\in\bar{C}$ and the following candidate Lyapunov function\footnote{In \cite{}, for consensus in $x \in \Re$, the Lyapunov function $V = \max(x_i) - \min(x_i)$ is studied.  Here we propose an equivalent Lyapunov but adapted to the domain of the unit vectors, namely the unit sphere.}
	%
	\begin{align}
		V = 1 - \nmb_i \tp \nmb_j \triangleq \underset{(k,l) \in V \times V }{\max}(1 - \nmb_k \tp \nmb_l),
	\end{align}
	%
	which is positive definite and zero if and only if $\bar{C} = \emptyset$, i.e. $V=0$ iff all unit vectors are the aligned. Given the initial condition for the Theorem, it follows that $V(0)<1$. The Lyapunov time derivative renders
	%
	\begin{align}
		\dot{V} 
		= & 
		- \nmb_j \tp \dot{\nmb}_i
		- \nmb_i \tp \dot{\nmb}_j
		\\
		= &
		-
		\underset{k \in \mathcal{N}_i}{\sum}
		f_{ik}'(\nmb_j,\nmb_k)
		(\nmb_j \tp\nmb_k ) \left(1 - \frac{\nmb_j \tp\nmb_i}{\nmb_j \tp\nmb_k}  \nmb_i \tp\nmb_k \right)
		\\
		& 
		-
		\underset{l \in \mathcal{N}_j}{\sum} 
		f_{jl}'(\nmb_j,\nmb_k)
		(\nmb_i \tp\nmb_l ) \left(1 - \frac{\nmb_i \tp\nmb_j}{\nmb_i \tp\nmb_l}  \nmb_j \tp\nmb_l \right)		
		\\
		\le &
		-
		\underset{k \in \mathcal{N}_i}{\sum}
		f_{ik}'(\nmb_j,\nmb_k)
		(\nmb_j \tp\nmb_k ) \left(1 -  \nmb_i \tp\nmb_k \right)
		\\
		& 
		-
		\underset{l \in \mathcal{N}_j}{\sum} 
		f_{jl}'(\nmb_j,\nmb_k)
		(\nmb_i \tp\nmb_l ) \left(1 -  \nmb_j \tp\nmb_l \right)			
		\\
		\le &
		-
		(1-V)
		\underset{k \in \mathcal{N}_i}{\sum}
		f_{ik}'(\nmb_j,\nmb_k)
		\left(1 -  \nmb_i \tp\nmb_k \right)
		\\
		& 
		-
		(1-V)
		\underset{l \in \mathcal{N}_j}{\sum} 
		f_{jl}'(\nmb_j,\nmb_k)
		\left(1 -  \nmb_j \tp\nmb_l \right)			
		\\		
		& 
		- k (1 - V) 
		\underset{k \in \mathcal{N}_i,l \in \mathcal{N}_j}{\max}
		\left(1 - \nmb_i \tp\nmb_k , 1 -  \nmb_j \tp\nmb_l\right)
		\\
		& \le 0					
	\end{align}
	%
	Since $\dot{V}$ is negative semi-definite, $V(t) \le V(0) < 1$ which means that $\min \, \nmb_i\tp \nmb_j > 0$ for all time. Additionally, since $\dot{V}$ is negative semi-definite and $V$ is lower bounded (by 0), it follows that $V$ must converge to a limit~\cite{slotine1991applied}. Suppose that $V$ converges to $\epsilon$ where $0<\epsilon \le V(0)<1$. Then
	%	
	\begin{align}
		\dot{V} \le - k (1 - \epsilon) 
		\underset{k \in \mathcal{N}_i,l \in \mathcal{N}_j}{\max}
		\left(1 - \nmb_i \tp\nmb_k , 1 -  \nmb_j \tp\nmb_l\right)
		<0,
	\end{align}
	%
	where the strict inequality at the right comes from the fact that that $(i,j) \in \bar{C}$ which by construction only includes pairs where either agent~$i$ or agent~$j$ has at least one neighbor that is not aligned with itself. As such, for a connected graph, $V$ can only converge to 0 which corresponds to a scenario where all agents are aligned, i.e. $\min \nmb_i\nmb_j = 1$.
\end{proof}
